Social Robots for Sleep Health: A Scoping Review

Poor sleep health is an increasingly concerning public healthcare crisis, especially when coupled with a dwindling number of health professionals qualified to combat it. However, there is a growing body of scientific literature on the use of digital technologies in supporting and sustaining individuals' healthy sleep habits. Social robots are a relatively recent technology that has been used to facilitate health care interventions and may have potential in improving sleep health outcomes, as well. Social robots' unique characteristics -- such as anthropomorphic physical embodiment or effective communication methods -- help to engage users and motivate them to comply with specific interventions, thus improving the interventions' outcomes. This scoping review aims to evaluate current scientific evidence for employing social robots in sleep health interventions, identify critical research gaps, and suggest future directions for developing and using social robots to improve people's sleep health. Our analysis of the reviewed studies found them limited due to a singular focus on the older adult population, use of small sample sizes, limited intervention durations, and other compounding factors. Nevertheless, the reviewed studies reported several positive outcomes, highlighting the potential social robots hold in this field. Although our review found limited clinical evidence for the efficacy of social robots as purveyors of sleep health interventions, it did elucidate the potential for a successful future in this domain if current limitations are addressed and more research is conducted.

==> tables/sleep_vars.tex <==
\begin{tabular}{!{\color{black}\vrule}>{\hspace{0pt}}m{0.55\linewidth}!{\color{black}\vrule}>{\hspace{0pt}}m{0.55\linewidth}!{\color{black}\vrule}>{\hspace{0pt}}m{0.10\linewidth}!{\color{black}\vrule}>{\vspace{3pt}\hspace{pt}}m{0.30\linewidth}!{\color{black}\vrule}>} 
\hline
\textbf{Construct Investigated} & \textbf{Data Collection Tool} & \textbf{Studies} & \textbf{Statistically Significant Effect? (Control/s)} \\ 
\hline
\hline
\textbf{\textit{Sleep-Duration-Related Outcomes}} & & & \\
\hline
\hline
Sleep duration~ & Questionnaire & \cite{oda} & Not applicable \\ 
\hline
 & Infrared sensor & \cite{mizuno} & Yes \\ 
\hline
Total time in bed & Sheet-shaped body vibrometer (SBV)~ & \cite{obayashi} & No \\ 
\hline
Time spent lying down & Actigraphy (SenseWear 8.0 Activity Armband)~ &  \cite{pu} & No \\ 
\hline
 & Actigraphy (SenseWear 8.0 Activity Armband)~ & \cite{moyle} & No \\ 
\hline
Sleep time (light sleep, deep sleep, very deep sleep)~ & Actigraphy (SenseWear 8.0 Activity Armband)~ & \cite{pu} & Yes \\ 
\hline
 & Actigraphy (SenseWear 8.0 Activity Armband)~ & \cite{moyle} & No \\ 
\hline
Nocturnal sleep hours & Questionnaire & \cite{tanaka} & Unclear \\ 
\hline
Actual sleep time & Actiwatch 4 (CamNTech) & \cite{thodberg} & No \\ 
\hline
Total sleep time (TST). & Sleep actigraph (ActiSleep+) & \cite{joranson} & Yes \\ 
\hline
\hline
\textbf{\textit{Sleep-Fragmentation-Related Outcomes}} & & & \\
\hline
\hline
\begin{tabular}[c]{@{}l@{}}\\Sleep efficiency~\end{tabular} & Sleep actigraph (ActiSleep+) & \cite{joranson} & Yes \\ 
\hline
 & Sheet-shaped body vibrometer (SBV)~ & \cite{obayashi} & No \\ 
\hline
 & Actiwatch 4 (CamNTech) & \cite{thodberg} & No \\
\hline
WASO (Wake after sleep onset) & Sleep actigraph (ActiSleep+) & \cite{joranson} & Yes \\ 
\hline
 & Sheet-shaped body vibrometer (SBV)~ & \cite{obayashi} & No \\ 
\hline
Fragmentation index & Actiwatch 4 (CamNTech) & \cite{thodberg} & No \\ 
\hline
Difficulty in maintaining sleep & 4-level scale & \cite{tanaka} &  \\ 
\hline
Total time leaving bed after sleep onset & Sheet-shaped body vibrometer (SBV)~ & \cite{obayashi} & No \\ 
\hline
Number of awakenings longer than 5 minutes (NA \textgreater{} 5) & Sleep actigraph (ActiSleep+) & \cite{joranson}  & Yes \\ 
 \hline
Time spent awake & Actigraphy (SenseWear 8.0 Activity Armband)~ & \cite{pu} & Yes \\ 
\hline
 & Actigraphy (SenseWear 8.0 Activity Armband)~ & \cite{moyle} & No \\ 
\hline
\hline
\textbf{\textit{Sleep-Inititation-Related Outcomes}} & & & \\
\hline
\hline
Bedtime & Infrared sensor & \cite{mizuno} & No \\
\hline
Difficulty initiating sleep~ & 4-level scale & \cite{tanaka} & Unclear \\ 
\hline
Sleep latency~ & Sheet-shaped body vibrometer (SBV)~ & \cite{obayashi} & No \\ 
\hline
\hline
\textbf{\textit{Wake-Up-Related Outcomes}} & & & \\
\hline
\hline
Wake-up time~ & Infrared sensor & \cite{mizuno} & Yes \\ 
\hline
Early morning awakening & 4-level scale & \cite{tanaka} & Unclear \\ 
\hline
Sleepiness (after wake-up) & \begin{tabular}[c]{@{}l@{}}Stanford Sleepiness Scale\end{tabular} & \cite{oda} & Yes \\
\hline
\textbf{\textit{Sleep-Hygiene-Related Outcomes}} & & & \\
\hline
\hline
Sleep Hygiene Score~ & 6-level scale & \cite{van2022interactive} & Yes \\ 
\hline
\end{tabular}

%JP: For the Construct Investigated column, change all "X X Related Outcomes to "X-X-Related Outcomes". Uncapitalize the following (except for the first letter): Total Time in Bed, Nocturnal Sleep Hours, Actual Sleep Time, Wake after sleep onset, Fragmentation Index, Sleep Latency, Wake-up Time, Early Morning Awakening. Remove the period after (TST). Add hyphen in "after wake-up".
%JP: For the Data Collection Tool column, uncapitalize the following (except for the first letter): Infrared Sensor, Sleep Actigraph. Add a space between "Actigraphy" and "(SenseWear" and "Actigraph" and "(ActiSleep+)".
%JP: Uncapitalize the A in "Not Applicable".
